Conditional Contrastive Learning for Improving Fairness in Self-Supervised Learning

Contrastive self-supervised learning (SSL) learns an embedding space that maps similar data pairs closer and dissimilar data pairs farther apart. Despite its success, one issue has been overlooked: the fairness aspect of representations learned using contrastive SSL. Without mitigation, contrastive SSL techniques can incorporate sensitive information such as gender or race and cause potentially unfair predictions on downstream tasks. In this paper, we propose a Conditional Contrastive Learning (CCL) approach to improve the fairness of contrastive SSL methods. Our approach samples positive and negative pairs from distributions conditioning on the sensitive attribute, or empirically speaking, sampling positive and negative pairs from the same gender or the same race. We show that our approach provably maximizes the conditional mutual information between the learned representations of the positive pairs, and reduces the effect of the sensitive attribute by taking it as the conditional variable. On seven fairness and vision datasets, we empirically demonstrate that the proposed approach achieves state-of-the-art downstream performances compared to unsupervised baselines and significantly improves the fairness of contrastive SSL models on multiple fairness metrics.

==> sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%

%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{At the end of the main text.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{At the end of the main text.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{All assumptions are stated in the main text.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{All the proofs are in the Supplementary material.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{In the Supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In the Supplementary material.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{In the Supplementary material.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In the Supplementary material.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{In the Supplementary material.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{In the Supplementary material.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{In the Supplementary material.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/fig_tex/algorithm.tex <==
% \begin{algorithm}[t]
% \caption{Conditional Contrastive Learning, PyTorch-like}
% \label{alg:code}
% \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
% \definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
% \lstset{
%   backgroundcolor=\color{white},
%   basicstyle=\fontsize{7.5pt}{7.5pt}\ttfamily\selectfont,
%   columns=fullflexible,
%   breaklines=true,
%   captionpos=b,
%   commentstyle=\fontsize{7.5pt}{7.5pt}\color{codeblue},
%   keywordstyle=\fontsize{7.5pt}{7.5pt}\color{codekw},
% }
% \begin{lstlisting}[language=python]
% # f: backbone + projection mlp
% # h: prediction mlp

% Sample z from Z
% for x in loader(z):  # load a minibatch x with n samples from z
%     x, y = aug(x), aug(x)  # augmentation
%     z1, z2 = f(x1), f(x2)  # encoder

%     L = InfoNCE(z1, z2)   # loss

%     L.backward()  # back-propagate
%     update(f, h)  # SGD update
% \end{lstlisting}
% \end{algorithm}

% Add algorithmic procedure. % https://proceedings.neurips.cc/paper/2021/file/64ff7983a47d331b13a81156e2f4d29d-Paper.pdf

==> sections/fig_tex/embedding.tex <==
% \begin{figure}[h]%
%     \centering
%     \subfloat[\centering Embedding space of contrastive SSL without mitigation ]{{\includegraphics[width=0.45\linewidth]{sections/fig/cl.png} }}%
%     \qquad
%     \subfloat[\centering Conditional Contrastive Learning ]{{\includegraphics[width=0.45\linewidth]{sections/fig/conditional.png} }}%
%     \caption{Add UTK; Remove everything and contain only the points. Embedding spaces of ordinary contrastive SSL vs. Conditional Contrastive Learning using t-SNE. The vector embeddings of two gender groups are visually separated in the ordinary contrastive SSL, while the embeddings learned via Conditional Contrastive Learning makes it very hard to separate both groups.}%
%     \label{fig:embedding}%
% \end{figure}


==> sections/fig_tex/intro-unfair.tex <==
\begin{wrapfigure}{r}{0.45\linewidth}
\centering
\includegraphics[width=0.6\linewidth]{sections/fig/figure1_new.png}
\caption{\small A demonstration of contrastive pre-training yielding unfairer results on the attractiveness task of the CelebA dataset. We train two ResNet-18 models~\citep{he2016deep}, one with contrastive pre-training then fine-tuning \citep{he2020momentum}, and one with supervised training. Both models have the same architecture and training hyperparameters. The difference of equality of opportunity ($\Delta_{EOpp}$) between the female and the male group is much larger in contrastive pre-training ($31.1\%$) than its supervised counterpart ($8.0\%$), suggesting that contrastive pre-training produces unfairer predictions.}
\label{fig:unfair}
\end{wrapfigure}

==> sections/fig_tex/method.tex <==
% \begin{wrapfigure}{l}{0.45\linewidth}
% \centering
% \includegraphics[width=0.8\textwidth]{sections/fig/method.png}
% \caption{\small \textbf{CCL framework}. We first sample from the sensitive attribute $z \sim Z$ (for instance, sample from gender, resulting female or male). A image batch will be sampled from the same $z$, i.e., all images in the batch have the same gender. Two augmented views of each images are then created, and the rest follows standard contrastive SSL frameworks like SimCLR \citep{chen2020simple}. Using images from the same $Z=z$ makes it harder for the model to leverage the sensitive information $Z$ to distinguish positive and negative pairs.}
% \vspace{-2mm}
% \label{fig:method}
% \end{wrapfigure}

\begin{figure}
\centering
\includegraphics[width=0.35\textwidth]{sections/fig/method.png}
\caption{\small \textbf{CCL framework}. We first sample from the sensitive attribute $z \sim Z$ (for instance, sample from gender, resulting female or male). A image batch will be sampled from the same $z$, i.e., all images in the batch have the same gender. Two augmented views of each images are then created, and the rest follows standard contrastive SSL frameworks like SimCLR \citep{chen2020simple}. Using images from the same $Z=z$ makes it harder for the model to leverage the sensitive information $Z$ to distinguish positive and negative pairs.}
\vspace{-2mm}
\label{fig:method}
\end{figure}

==> sections/table/fair_full.tex <==
\begin{table*}[ht]
\centering
\caption{\label{tab:results_node}Ranking results for multi-step prediction in latent space. Highest (mean) scores in \textbf{bold}.}

\begin{adjustbox}{center,width=0.9\linewidth}
\begin{tabular}{lllcccccc}
\toprule
  & & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Fairness} \\ \cmidrule(lr){4-6} \cmidrule(lr){7-9}
&&Model &Accuracy $(\uparrow)$ & AP $(\uparrow)$ & ROC $(\uparrow)$ & $\Delta_{DP}\,(\downarrow)$ & $\Delta_{EO}\,(\downarrow)$ & $\Delta_{{EO}_{PP}}\,(\downarrow)$      \\ \midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{ADULT}}}} & Unsupervised (InfoNCE)& {83.1} &
 &
 & 
 0.21 &
0.41 &

\\
&&-- \citet{moyer2018invariant} & 75.2 & & & & & \\
&&--  LAFTR \citep{madras2018learning} & 84.0 & - & - & 0.163 & 0.030 & 0.026 \\
&&-- LMIFR \citep{song2019learning} &  &  &  &  & &

\\
% &&-- \citet{ferrari2021addressing} && & & \\
% &&-- \citep{akash2021learning} & & & & \\
% &&-- \citet{shen2022fair} & & & & \\
% &&-- \citep{Fair Representations by Compression} & & & & \\
% \hdashline

&&-- LCIFR \citep{ruoss2020learning} & 83.0 & & & & & \\
&&-- \citet{ragonesi2021learning} & & & & & &  \\

&&-- {\color{red} \textbf{Very similar work}} \citet{gupta2021controllable} & 84.0 & & & 0.16 & & \\

&&-- \citet{lee2020maximal} & 71.6 & & & & 0.05 & \\
&&-- \citet{balunovic2021fair} & 80.0 & & & 0.11 & & \\
&&-- \citet{ferrari2021addressing} & & & & & & \\

&&-- \citet{mehrabi2021attributing} & & & & & & \\
&&-- \citet{sattigerichi} & & & & & & \\
&&-- \citep{akash2021learning} & & & & & & \\
&&-- \citep{shen2022fair} & & & & & & \\
&&-- \citep{lokhande2022towards} & & & & & & \\
&&-- \citep{Fair Representations by Compression} & & & & & & \\
&&-- \bf CInfoNCE & \bf 85.4 &  &  & 0.12 & 0.25  & \\
% \midrule
% &&\bf Supervised & \\
% &&-- Fair-Mixup \citep{chuang2021fair}  & 76.4  & 0.065 & 0.025  & - \\
% &&-- \citet{gupta2021controllable} & 84.0& 0.16 & & \\

% &&-- \citet{sarhan2020fairness} & & & & \\
% &&-- \citet{jaiswal2020invariant} & & & & \\
% &&-- \citet{sadeghi2020imparting} & & & & \\
% &&-- \citet{zhu2021learning} & & & & \\
% &&-- \citet{cerrato2022fair} & & & & \\
% &&-- CHI2MI \citep{sattigerichi} & 84.0 & - & - & 0.02 \\
% &&-- \citet{mehrabi2021attributing} & 84.5 & 0.13 & & \\
% % &&-- \citep{lokhande2022towards} & & & & \\


&&Supervised (Fair-Mixup \citep{chuang2021fair})  & 76  &  & & 0.06 & 0.023  & \\
&&-- \citet{sarhan2020fairness} & & & & & & \\
&&-- \citet{jaiswal2020invariant} & & & & & & \\
&&-- \citet{sadeghi2020imparting} & & & & & & \\
&&-- \citet{zhu2021learning} & & & & & & \\
&&-- \citet{cerrato2022fair} & & & & & & \\


\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{COMPAS}}}} &Unsupervised (InfoNCE) &
71.2 & & & 0.10 & 0.22 &
\\
&&-- \bf CInfoNCE & 70.8 &  &  & 0.08 & 0.13  & \\
&&-- \citet{lee2020maximal} & 66.0 & & & & 0.2 & \\
&&-- \citet{balunovic2021fair} & 67.0 & & & 0.10 & & \\
&&-- \citet{grari2021learning} & & & & & & \\
&&-- \citet{sattigerichi} & & & & & & \\
&&-- \citep{Fair Representations by Compression} & & & & & & \\

\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{CRIME}}}}&Unsupervised (InfoNCE) &
82.1 & & & 0.50 & 0.53 &
\\
&&-- \bf CInfoNCE &  82.6 &  &  & 0.21 & 0.22  & \\
&&-- LCIFR \citep{ruoss2020learning} & 84.4 & & & & & \\
&&-- \citet{balunovic2021fair} & 82.5 & & & 0.5 & & \\
&& & & & & & & \\
&& & & & & & & \\

\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{GERMAN}}}}&Unsupervised (InfoNCE) &
72.5 & & & 0.25 & 0.38 &
\\
&&-- \bf CInfoNCE & 74.3 &  &  & 0.09 & 0.25  & \\
&&-- \citet{mehrabi2020exacerbating} & & & & & & \\
&&-- \citet{sattigerichi} & & & & & & \\
&&-- \citet{cerrato2022fair} & & & & & & \\
&&-- \citet{liu2021fairness} & & & & & & \\
&& & & & & & & \\

\midrule
\parbox[t]{0.1mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{LAW}}} & \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{SCHOOL}}} 
&Unsupervised (InfoNCE) &
83.0 & & & 0.08 & 0.2 &
\\
&&-- \bf CInfoNCE & \bf 84.8 &  &  & 0.05 & 0.15  & \\
&&-- LCIFR \citep{ruoss2020learning} & 84.4 & & & & & \\
&&-- \citet{balunovic2021fair} & 84.8 & & & 0.08 & & \\



\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> sections/table/full.tex <==
\begin{table}[H]
\centering
\caption{TODOTODOTODOTODOTODOTODOTODOTODOTODOTODOTODOTODOTODOTODOTODOTODOTODOAccuracies and fairness metrics results on seven datasets. Some scores are read from the figures in the original papers. Results not significantly worse than the best are bold. CCL has better accuracy than existing unsupervised and self-supervised in four out of the five datasets, and exhibits better or close-to-the-best fairness measurements on almost all datasets.}

\begin{adjustbox}{center,width=0.85\linewidth}
\begin{tabular}{lllcccc}
\toprule

% Double check EOPP scores and LCIFR scores
%   & & & \multicolumn{1}{c}{Accuracy} & \multicolumn{3}{c}{Fairness} \\ \cmidrule(lr){4} \cmidrule(lr){5-7}
&&Model &Accuracy (\%) $(\uparrow)$ & $\Delta_{DP}\,(\downarrow)$ & $\Delta_{EO}\,(\downarrow)$ & $\Delta_{{EO}_{PP}}\,(\downarrow)$      \\ 
\midrule

\multicolumn{7}{c}{Fairness Dataset Experiments} \\
\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{ADULT}}}} & \bf Unsupervised\\
&&--  LAFTR \citep{madras2018learning} & 84.0 & 0.163 & \bf 0.030 & \bf 0.026 \\
% &&-- LCIFR \citep{ruoss2020learning} & 83.3 & \bf 0.102 & 0.043 & 0.036 \\
% Need to double check this LCIFR number
&&-- \citet{ragonesi2021learning} & 85.0 & - & \bf 0.030 & -  \\
&&-- DTM \citep{lee2020maximal} & 71.6 & -& 0.050 & -\\
&&-- FNF \citep{balunovic2021fair} & 80.0 & \bf 0.110 & - & - \\
% &\\
&&\bf Self-Supervised & \\
&&-- SimCLR \citep{chen2020simple} & 83.1 & 0.210 & 0.410 & 0.320\\
&&-- FairMixRep \citep{chakraborty2020fairmixrep}  & 85.0 & 0.172 & - & - \\
&&-- \bf CCL (Ours) & \bf 85.4 & \bf 0.110 & 0.070  & 0.090 \\


\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{COMPAS}}}} &\bf Unsupervised \\
&&-- DTM \citep{lee2020maximal} & 66.0 & - & 0.200 & - \\
&&-- FNF \citep{balunovic2021fair} & 65.0 & 0.240 & - & - \\
&&\bf Self-Supervised & \\
&&-- SimCLR \citep{chen2020simple}  & \bf 71.2 & 0.103 & 0.227 & 0.134 \\
&&-- \bf CCL (Ours) & \bf 71.0& \bf 0.080 & \bf 0.132  & \bf 0.081 \\

% &&Supervised (Fair-Mixup \citep{chuang2021fair})  & 76  & 0.06 & 0.023  & \\
% &&-- CHI2MI \citep{sattigerichi} & 0.83 & - & - & 0.10\\


\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{CRIME}}}}&\bf Unsupervised&\\
% Need to double check this LCIFR number

&&-- LCIFR \citep{ruoss2020learning} & 84.4 & 0.443 & 0.314 & 0.212 \\
&&-- FNF \citep{balunovic2021fair} & 82.5 & 0.540 & - & - \\
&&\bf Self-Supervised\\
&&-- SimCLR \citep{chen2020simple} & 82.1 & 0.50 & 0.530 & 0.383 \\
&&-- \bf CCL (Ours) & \bf 82.6 & \bf 0.211 & \bf 0.224  & \bf 0.183 \\

\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{GERMAN}}}}& \bf Unsupervised\\
% CHeck all equalized odds
&&-- LCIFR \citep{ruoss2020learning} & 73.1 & 0.102 & 0.080 & 0.063 \\
&&-- FairMixRep \citep{chakraborty2020fairmixrep}  & 71.8 & 0.089 & - & - \\

&&-- \citet{ragonesi2021learning} & 74.0 & - & \bf 0.060 & -  \\
&&\bf Self-Supervised\\

&&-- SimCLR \citep{chen2020simple}   & 72.5 &0.250 & 0.382 & 0.195 \\
&&-- \bf CCL (Ours) & \bf 74.3 & \bf 0.083 & 0.128  & \bf 0.062 \\

\midrule
\parbox[t]{0.1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{LAW}}} & \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{SCHOOL}}} &
\bf Unsupervised\\ 
&&-- LCIFR \citep{ruoss2020learning} & 84.4 & 0.110 & 0.180 & 0.070 \\
&&-- FNF \citep{balunovic2021fair} & 84.6 & \bf 0.050 & - & - \\
&&\bf Self-Supervised\\
&&-- SimCLR \citep{chen2020simple}   & 83.6 & 0.086 & 0.212 & 0.110 \\
&&-- \bf CCL (Ours) & \bf 84.8 & \bf 0.051 & \bf 0.153  & \bf 0.056\\

\midrule 
\multicolumn{7}{c}{Vision Dataset Experiments} \\ 
\midrule
\parbox[t]{0.1mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{CELEBA}}} & \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{ATTRACTIVE}}} &
\bf Unsupervised\\ 
&&-- MFD \citep{jung2021fair} & 80.2 & - & \bf 0.050 & - \\
&&-- \citet{balunovic2021fair} & 79.4 & - & 0.238 & - \\
&&-- \citet{morales2020sensitivenets} & 77.7 & - & 0.070 & - \\
&&\bf Self-Supervised\\
&&-- SimCLR \citep{chen2020simple}   & 81.7 & 0.277 & 0.212 & 0.110 \\
&&-- \bf CCL (Ours) & \bf 82.1 & \bf 0.202 & 0.101  & \bf 0.048\\
% https://arxiv.org/pdf/2106.04411.pdf
\midrule
\parbox[t]{0.1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{CELEBA}}} & \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{WAVY HAIR}}} &
\bf Unsupervised\\ 
&&-- FactorVAE \citep{kim2018disentangling} & 64.5 & - & 0.388 & 0.288 \\
&&-- FFVAE \citep{creager2019flexibly} & 61.0 & - & 0.211 & 0.154 \\
&&\bf Self-Supervised\\
&&-- SimCLR \citep{chen2020simple}   & \bf 67.7 & 0.403 & 0.355 & 0.210 \\
&&-- \bf CCL (Ours) & \bf 67.7 & \bf 0.202 & \bf 0.189  & \bf 0.102\\

\midrule
\parbox[t]{0.1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{CELEBA}}} & \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{SMILE}}} &
\bf Unsupervised\\ 
&&-- \citet{morales2020sensitivenets} & 88.4 & - & 0.060 & - \\

&&\bf Self-Supervised\\
&&-- SimCLR \citep{chen2020simple}   & 89.3 & 0.102 & 0.142 & 0.078 \\
&&-- \bf CCL (Ours) & \bf 89.7 & \bf 0.086 & \bf 0.060  & \bf 0.053\\

\midrule
\parbox[t]{0.1mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{UTK}}} & \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{GENDER}}} &
\bf Unsupervised\\ 
&&-- AD \citep{zhang2018mitigating} & 74.7 & - & 0.204 & - \\
&&-- MFD \citep{jung2021fair} & 74.7 & - & 0.178 & - \\
&&\bf Self-Supervised\\
&&-- SimCLR \citep{chen2020simple}   & 78.0 & 0.335 & 0.421 & 0.287 \\
&&-- \bf CCL (Ours) & \bf 78.5 & \bf 0.191 & \bf 0.156  & \bf 0.089\\

\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:fair}

\end{table}


==> sections/table/speech.tex <==
\begin{table}[t!]
%\vspace{-3mm}
    \begin{center}
        % \scalebox{0.7}{
        \begin{tabular}{{0.3\textwidth}{0.26\textwidth}{0.26\textwidth}}
            \toprule
            Objective & Phoneme Classification (\uparrow) & Speaker Classification (\downarrow) \\
            \midrule \midrule 
            \multicolumn{3}{c}{\it Unconditional Self-supervised Learning} \\ \midrule \midrule
             InfoNCE & $63.6_{\pm 0.12}$ & $93.4_{\pm 0.18}$ \\
             \midrule \midrule
             \multicolumn{3}{c}{\it Conditional Self-supervised Learning ($Z=$ Speaker ID)} \\ \midrule \midrule
             C-InfoNCE (ours) & $64.3_{\pm 0.13}$ & ${71.2}_{\pm 0.14}$ \\ [1mm]
             WeaC-InfoNCE (ours) & $63.8_{\pm 0.12}$ & $72.0_{\pm 0.13}$ \\
             \midrule \midrule
             \multicolumn{3}{c}{\it Conditional Self-supervised Learning ($Z=$ Sequence ID)} \\ \midrule \midrule
             C-InfoNCE (ours) & ${64.5}_{\pm 0.11}$ & $71.6_{\pm 0.12}$ \\ [1mm]
             WeaC-InfoNCE (ours) & $64.2_{\pm 0.13}$ & $72.3_{\pm 0.13}$ \\
            \bottomrule
        \end{tabular}%}
    \end{center}
\caption{ \small Accuracy (\%) for LibriSpeech-100h phoneme and speaker classification results using self-supervised representations (conditional versus unconditional contrastive learning methods). We consider the meta information including the speaker and sequence ID as the conditioned variable $Z$.
%,where conditioning a variable removes the effect from this variable. We find removing such meta information in the speech representations results in better Phoneme Classification and worse Speaker Classification. A possible explanation is that the speaker and sequence ID information is irrelevant to Phoneme Classification but relevant to Speaker Classification.
}
\label{tab:speech}
\end{table}

==> sections/table/vision_full.tex <==
\begin{table*}[ht]
\centering
\caption{\label{tab:results_node}Ranking results for multi-step prediction in latent space. Highest (mean) scores in \textbf{bold}.}

\begin{adjustbox}{center,width=0.9\linewidth}
\begin{tabular}{lllcccccc}
\toprule
  & & & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Fairness} \\ \cmidrule(lr){4-6} \cmidrule(lr){7-9}
&&Model &Accuracy $(\uparrow)$ & AP $(\uparrow)$ & ROC $(\uparrow)$ & $\Delta_{DP}\,(\downarrow)$ & $\Delta_{EO}\,(\downarrow)$ & $\Delta_{{EO}_{PP}}\,(\downarrow)$      \\ \midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Attractive}}}} & 
Unsupervised (InfoNCE) & 85.51  &  & & 0.51 & 0.62 & 0.26 \\
&&-- \bf CInfoNCE (Ours) & \bf 87.33 & & & 0.13 & 0.31 & 0.12\\
&&-- MFD \citep{jung2021fair} & 80.20 & & & 0.05 & - & - \\
&&-- \citet{seo2021unsupervised}($\Delta_{DP}=0$) & 77.90 & & & 0 & - & - \\
&&-- \citet{liu2021mutual} & & & & & & \\
&&-- \citet{smieja2020segma} & & & & & & \\
&&-- \citet{samragh2021unsupervised} & & & & & & \\
&&-- \citet{samragh2020private} & & & & & & \\
&&-- \citep{shen2022fair} & & & & & & \\
&&-- \citep{lokhande2022towards} & & & & & & \\
&&-- \citep{malekzadeh2021honest} & & & & & & \\

&&Supervised \citep{chuang2021fair} & 87.10 & & & 0.06 & 0.08 & - \\
&&-- \citet{seo2021unsupervised}($\Delta_{DP}=0$) &78.35  & & & 0 & -& -\\
&&-- \citet{zhu2021learning} & & & & & & \\
&&-- \citet{shen2022fair} & & & & \\



\midrule
\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Wavy hair}}}}&
Unsupervised (InfoNCE) & 93.21  &  & & 0.51 & 0.62 & 0.26 \\
&&-- \bf CInfoNCE (Ours) & \bf 97.22 & & & 0.08 & 0.08 & 0.07\\
&&-- \citet{seo2021unsupervised}($\Delta_{DP}=0$) & 79.89 & & & 0 & - & - \\
&&Supervised \citep{chuang2021fair} & 97.10 & & & 0.03 & 0.01 & - \\
&&-- \citet{seo2021unsupervised}($\Delta_{DP}=0$) &79.65 & & & 0 & -& -\\

\midrule

\multicolumn{2}{c}{\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Smile}}}}&
Unsupervised (InfoNCE) & 81.77  &  & & 0.31 & 0.52 & 0.33 \\
&&-- \bf CInfoNCE (Ours) & 84.32 & & & 0.30 & 0.33 & 0.21\\
&&-- \citet{seo2021unsupervised} ($\Delta_{DP}=0$) ??? & 92.08 & & & 0 & - & - \\
&&Supervised \citep{chuang2021fair} & 83.21 & & & 0.08 & 0.08 & - \\
&&-- \citet{seo2021unsupervised}($\Delta_{DP}=0$) &91.64  & & & 0 & -& -\\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> sections/trash.tex <==
%_---------------------------------------Introduction--------------------------------

% Empirically, contrastive pre-training exhibits these undesirable biases because they can pick up information from the sensitive attribute to distinguish positive from negative samples. We provide an illustrative example in Figure~\ref{fig:intro_illu} (left), where the model uses gender information as a useful discriminative factor to distinguish positive from negative samples that do not share the same gender, and generating an embedding space with gender bias. 

%This is indeed the case from our empirical observation (Section \ref{sec:behavior}) where the embedding space learned via contrastive SSL makes it easy to separate the female group from the male group, causing potential bias issues in downstream tasks. 

%A direct solution is to remove the sensitive attributes when pre-training. However, this may not be optimal because many attributes could still be related to the sensitive attributes (for example, occupation often correlates with gender). Furthermore, in real-world datasets like CelebA \citep{liu2015faceattributes}, there is no straightforward way to remove sensitive attributes (e.g., hard to remove all gender-indicating features in the image, like hair style or mustache).

%We illustrate a demonstration on CelebA \citep{liu2015faceattributes} dataset in Figure \ref{fig:unfair}. When we compare the differences of equality of opportunity ($\Delta_{EOpp}$, measuring the differences of true positive rates between subgroups), the model trained via contrastive pre-training has much higher $\Delta_{EOpp}$ than the supervised counterpart (a whopping $23.1\%$ gap), indicating that the model learned by contrastive pre-training yields unfairer predictions. Such phenomenon exposes a fundamental blind spot of existing contrastive SSL methods, raising concerns for potential social harm on different downstream tasks \citep{liu2020self}.


%Contrastive SSL methods often first choose a data point as an anchor, and then define data related to the anchor as the positive samples, and data unrelated to the anchor as the negative samples. For example, given an image of dog as the anchor, the positive samples could be augmented variants of the dog image, while negative samples could be random images in the dataset. An encoder will map the anchor point, the positive samples and the negative samples to an embedding space. A contrastive objective function then maximizes the similarity of embeddings between the anchor and the positive samples, meanwhile minimizing the similarities of embeddings between the anchor and the negative samples \citep{oord2018representation}. Recent work considers the contrastive objective as maximizing the mutual information between the positive sample and the anchor \citep{tschannen2019mutual, tsai2021multiview}. After this phase of self-supervised training often termed as contrastive pre-training, supervised fine-tuning is performed by freezing the encoder and finetuning a small net on top of the encoder with labels to evaluate the representation quality of the encoder \citep{chen2020big}.

% Add figure like this: https://proceedings.neurips.cc/paper/2021/file/64ff7983a47d331b13a81156e2f4d29d-Paper.pdf

% Clear explanation: https://proceedings.neurips.cc/paper/2020/file/f490c742cd8318b8ee6dca10af2a163f-Paper.pdf

% Clear writing like the ICML paper.

% A possible explanation is that the contrastive pre-training takes advantage of the given sensitive attributes from the dataset (for example, gender, race or personal identity information) to discriminate positive samples against negative samples, causing the model to explicitly contain information from the sensitive attributes. For example, if gender attribute is available, the model may use the gender attribute as a discriminative feature to distinguish the anchor points from negative points that do not share the same gender. This is indeed the case from our empirical observation, as illustrated in Figure \ref{fig:embedding}, where the embedding space learned via contrastive SSL makes it very easy to separate the female group from the male group, causing potential fairness issues. A direct solution is to remove the sensitive attributes when pre-training. However, this may not be optimal because many attributes could still be related to the sensitive attributes (for example, occupation often correlates with gender). Furthermore, in real-world datasets like CelebA \citep{liu2015faceattributes}, there is no straightforward way to remove sensitive attributes (e.g., hard to remove all gender-indicating features in the image, like hair style or mustache).

% , generating an embedding space with gender biases and
% models can leverage information from the sensitive attribute (gender) to distinguish positive from negative samples. 
% Sensitive attributes based on underrepresented subgroups, such as gender or ethnicity, are present in many datasets (Mehrabi et al., 2019). Without careful treatment, representations learned by contrastive method will incorporate these attributes during pre-training, making unfair decisions towards certain subgroups on downstream tasks.
% On the contrary, a fair representation should not include information from sensitive attributes

% contrastive pre-training can fail miserably on fairness. In Section \ref{sec:behavior}, we show that existing contrastive SSL methods yield biased representations and result in much larger differences in statistical parity \citep{feldman2015certifying}, equalized odds \citep{hardt2016equality}, and equality of opportunity \citep{hardt2016equality} than its supervised counterparts. The wide usage of contrastive SSL models in real-world tasks can potentially amplify these biases and discriminate against different demographic groups, causing danger and significant challenges in downstream tasks even more so than supervised models.

%  compared to the case of conventional contrastive learning where negative pairs can be distinguished by using gender-related information. pull together positive pairs and push away negative pairs, because the model gender-related information is less helpful to push away . 

% \citep{oord2018representation} objective, the new objective maximizes a lower bound of conditional mutual information within representations (similar to work which relates contrastive SSL to maximizing a lower bound of mutual information), while explicitly excluding information from the sensitive attribute.

% first  the sensitive attribute whose information we want to reduce as the conditioning variable, and samples negative pairs from the product of conditional marginal distributions during contrastive pre-training. Taking gender as the example of sensitive attribute, the distributions will be conditioned on gender, and all positive and negative pairs within a batch will have the same gender.
%instead of pushing away the embeddings of two random images, CCL pushes away the embeddings of images from the same gender, which is a harder task. 

%This is a sampling alteration, so such a framework can be adapted to existing contrastive objectives with minimal effort. 

% From Paul - can we illustrate the argument below with a figure

% This paragraph is too long
% {\color{red} This paragraph needs help from LP and Paul.} Alternatively, we provide an intuitive view of why our method should work, For example, if gender is the sensitive attribute, each batch only contains images from the same gender. As a result, the model is less likely to use superficial gender-related information, such as if a person has beard or wear lipsticks, to distinguish positive and negative pairs. This is because all the positive and negative pairs share the same gender and will likely share those superficial attributes. For instance, if the batch is from the female group, most female celebrities in CelebA dataset wear lipstics, making this feature (``wear lipsticks'') less likely to be picked up during contrastive learning. Compared to conventional contrastive SSL, CCL will more likely to use gender-independent features to to distinguish positive from negative pairs. By using gender-independent information rather than superficial gender-related information, CCL can achieve better fairness, while still maintaining good representation quality by using a contrastive SSL pre-training.

%away the embeddings of images from the same gender while conventional contrastive SSL pushes away the embddings of images from mixed genders, and 

%-------------------------Related---------------------------------
% instead of capturing more information between the data views. The final objective in \citet{sordoni2021decomposed} is a lower bound of mutual information, while the objective in this work is a lower bound of conditional mutual information. Also, this work

%To obtain bounds for conditional MI \citet{sordoni2021decomposed} approximates conditional distributions with variational approximations. 

